QCP: A Practical Separation Logic-based C Program Verification Tool

As software systems increase in size and complexity dramatically, ensuring their correctness, security, and reliability becomes an increasingly formidable challenge. Despite significant advancements in verification techniques and tools, their practical application to complex, real-world systems is often hindered by critical gaps in both automation and expressiveness. To address these difficulties, this paper presents \textbf{Qualified C Programming Verifier (QCP)}, a novel verification tool that integrates annotation-based automatic verification with interactive proving using Rocq. QCP employs symbolic execution and a separation logic entailment solver to automatically discharge many verification obligations, while deferring more complex obligations to Rocq for manual proof. Furthermore, QCP includes a VS Code extension designed to enhance proof efficiency and support a deeper understanding of both the program behavior and verification outcomes.

==> Approach.tex <==
\section{New Features in QCP}\label{sec::features}

As mentioned in the Section~\ref{sec::examples}, we find it not convenient enough for verifying real-world C programs only depending on features such as \lstinline{open}/\lstinline{close} and lemma functions. We will introduce our solutions, i.e. QCP's major features.

\input{Features/PartialAssertion}

\input{Features/Multispec}

\input{Features/ControlAssertion}


\input{Features/Multibranch}

%\input{Features/Multiinv}

\subsection{Discussion}

Following the introduction of our features, we address several potential questions that may arise.

\paragraph{Multi-spec vs. Assertion transformation before function calls}

One may argue that all assertion transformations before function calls could be handled by writing corresponding specifications for each case using the \lstinline{multi-spec} feature. While this is indeed possible, it is not always necessary. If such cases occur frequently or involve complex assertion transformations, we recommend using multi-spec for reusability and to reduce the overall transformation burden. Conversely, if such cases are rare and involve relatively simple transformations, we suggest using assertion transformation commands for direct modification.

\paragraph{Multi-inv with partial assertions vs. Invariants with full assertions}

Upon reviewing our example of \lstinline{multi-inv}, one may question whether writing full assertion-based invariants would be simpler. While this may appear true for simpler programs, as program complexity increases, the difficulty of writing full assertions grows correspondingly and often becomes impractical. Our \lstinline{multi-inv} design facilitates a clearer understanding of loop structures for the verifier and aligns the proof process more closely with the program’s structure.










==> Features/ControlAssertion.tex <==
\subsection{Declarative annotations}\label{DOA}

As mentioned in Section~\ref{sec::examples}, separation logic symbolic execution requires appropriate assertion transformations. We observe that the most convenient and natural transformation approach depends on the specific context. To address this, we provide flexible mechanisms to support such transformations, ensuring that symbolic execution can proceed effectively even in the presence of complex user-defined predicates. 

\paragraph{Full Assertion / Partial Assertion}
The most direct method is to write a new, complete assertion that explicitly describes the transformed goal. This generates a verification condition (VC) that must be manually discharged by the user. As stated in Section~\ref{fea::pasrt}, users are also permitted to write partial assertions.

\paragraph{Which Implies}
The \lstinline{which implies} command combines the frame rule and consequence rule from separation logic to support controlled assertion transformations. In our implementation, the solver partitions the current program state into two components based on memory permissions: the modified portion (to be transformed) and the residual frame (unchanged and preserved via the frame rule). The modified portion is replaced with the user-provided postcondition specified in \lstinline{which implies}, while the residual frame remains unchanged.

\begin{figure}[!htp]
  \centering
  \vspace{-1.0em}
  \inputminted[frame=lines,linenos]{c}{Figures/LOS_ListTailInsertFull.list}
  \vspace{-1.0em}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{Annotations for \lstinline{LOS_ListTailInsert}. Here we use \lstinline{which implies} (In line 9-15) to partition the memory of \lstinline{store_dll}.}
  \vspace{-1.0em}
  \label{fig:LosListTailInsertFull}
\end{figure}

In the example shown in Figure~\ref{fig:LosListTailInsert}, we utilize \lstinline{which implies} to complete the corresponding assertion transformation, thereby enabling the function call. Figure~\ref{fig:LosListTailInsertFull} illustrates the use of \lstinline{which implies} in this context. And the annotations of \lstinline{LOS_ListHeadInsert} can be seen in Appendix~\ref{appendixB}.

Here, we use the definitions \lstinline{dllseg_shift}, whose definition is shown in Figure~\ref{fig:dllseg_shift}. This represents the residual memory permission structures of \lstinline{store_dll} after the red-highlighted parts have been removed. The red-highlighted parts are written in the post of \lstinline{which implies}. The formal definition is provided below.

\begin{lstlisting}
dllseg_shift(px,py,l) := px == py && l == nil && emp || 
                       exists x a l', l == cons(a, l') && 
                       x == snd a && x -> pstData == fst a && 
                       x -> pstPrev == px && px -> pstNext == x &&
                       dllseg_shift(x, py, l')
\end{lstlisting}

\begin{figure}[!htp]
  \centering
  \vspace{-3.0em}
  \includegraphics[width=1\textwidth]{Figures/DLL_shift.png}
  \vspace{-1.0em}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{The definition of predicate \lstinline{dllseg_shift}. This predicate represents the memory structure depicted by the white area in the figure, which corresponds to the \lstinline{store_dll} structure excluding the red-highlighted portions.}
  \vspace{-1.0em}
  \label{fig:dllseg_shift}
\end{figure}




% \paragraph{Strategy-Based Operation}
% Many transformations on (co)inductively defined predicates are folding and unfolding. We support specifying generalized operational rewriting strategies in Stellis and apply them when appropriate. In this way, we support not only single-layer predicate unfolding and folding, similar to VeriFast's \lstinline{open} and \lstinline{close}, but also multi-layer predicate unfolding and folding in complex scenarios with a single command. We associate each strategy in Stellis with a defined scope. Users can then invoke the strategies within a specific scope using the \lstinline{do scope_name} command to perform the corresponding transformation.



==> Features/Multibranch.tex <==
\subsection{Multi-branch}

From now on, we call each clause in the disjunction a \emph{branch}, since branches in program states often result from branched execution. Sometimes branches are harmless, such as the code fragment in the following, where they are broken apart ultimately; sometimes, not. We provide mechanisms to manipulate branches.

\begin{lstlisting}
/*@ Assert p == q && store_dll(p,l1) * store_dll(r,l3) || 
           store_dll(p,l1) * store_dll(q,l2) * store_dll(r,l3) */
swap(p,q);
swap(p,r);
\end{lstlisting}

We require users to assign names to branches beforehand because designating branches by indices becomes unreliable when external tools may reorder them. Additionally, we deliberately avoid automatically generating names, unlike typical proof assistants. Although writing such annotations is straightforward with the support of our development environment, this approach is prone to issues during modifications. By design, we name branches based on trivial facts, meaning without relying on custom automation.

\begin{lstlisting}
￥\textcolor{gray}{/* the first case names the first branch, the second names the rest. */}￥
/*@ Branch name 2dlist: p == q; 3dlist */
\end{lstlisting}

% The best we can hope for is a specification like this:
In this example, it is clear that the result of \lstinline{swap(p, q)} differs significantly between the two branches, which further affects the outcome of \lstinline{swap(q, r)}. If we use the following specification, it will inevitably lead to significant challenges, as we would need to eliminate many impossible cases.

\begin{lstlisting}
/*@ With u v
    Require *p == u && *q == v || p == q && *p == u
    Ensure  *p == v && *q == u || p == q && *p == u */
\end{lstlisting}

By combining multi-specification and multi-branch support, we can write the following annotations, which are much more concise and clear.

\begin{lstlisting}
swap(p,q) /*@ where (eq_spec) $ 2dlist (neq_spec) $ 3dlist */;
swap(q,r) /*@ where (eq_spec) $ 2dlist (neq_spec) $ 3dlist */;  
\end{lstlisting}

Here, we use \lstinline{where} to specify the name of the particular specification and \lstinline{$ name} to denote the specific branch name. This allows different branches to execute distinct symbolic execution processes. Assertion control commands, namely \lstinline{which implies}, \lstinline{do}, and asserting, can be parameterized by branches involved. Other branches are kept as-is.

\paragraph{To change the number of branches:}

In scenarios where it is necessary to perform case analysis on a logical variable to determine the unfolding strategy of a predicate, we provide the \lstinline{Destruct} command to facilitate such classifications.

Additionally, to manage the complexity that may arise from an excessive number of branches, we offer the \lstinline{Branch join} command to merge branches and the \lstinline{Branch clear} command to eliminate unnecessary branches.

Due to space constraints, we do not elaborate on the specific usage of these features here. For detailed information, please refer to the documentation accompanying our artifact. In summary, these features enhance control over assertions during the verification process.

\paragraph{For loop invariants:}

Regarding loop invariants, since we permit the use of partial assertions within the loop invariant section, multiple branches can introduce significant complexity. When dealing with differing partial assertions, how should the branches within the invariant correspond to external branches? If the partial assertions are identical across branches, should the frames derived from different branches remain distinct, or should one be selected?

Moreover, in cases such as the invariant with multiple cases illustrated in Figure~\ref{fig:rbt}, how can we describe the evolution of the assertion corresponding to the invariant throughout the loop execution?

We introduce the \lstinline{multi-inv} feature to address these challenges. Specifically, we allow users to specify the entry point of each assertion upon entering the loop. In Figure~\ref{fig:rbt_new}, we demonstrate how this feature facilitates the verification of the aforementioned program.

At the beginning of the loop, we define loop invariants for two branches, corresponding to the previously mentioned scenarios. For assertions entering the loop, we use the \lstinline{with} clause to indicate that all branches fall into the standard \lstinline{RBT_inv} branch. After line 16, as the state transitions to the loop's termination phase, we only need to specify that the \lstinline{RBT_inv} branch transitions to the \lstinline{Loop_exit} branch. For other cases, the \lstinline{RBT_inv} branch loops back to itself, thus requiring no additional annotations. 

\wxw{For the \lstinline{Loop_exit} branch, since it never re-enters the loop body, our approach leverages the partial assertion feature. This allows QCP to automatically compute branch-specific assertions without requiring complete full assertions to be manually specified.}

\begin{figure}[t]
  \centering
  \inputminted[frame=lines,linenos]{c}{Figures/rbt_new.list}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{A red-black tree example utilizing the \lstinline{multi-inv} feature.}
  \label{fig:rbt_new}
\end{figure}


==> Features/Multiinv.tex <==
\subsection{Multi-invariant}

% Our solver solves queries of the form $P \vdash Q\;*\;?$ where $P$ and $Q$ are disjunction-free. This means that we have no problem solving $P_1 \lor P_2 \vdash Q\;*\;?_1 \lor Q \;*\; ?_2$ but we do have problems solving $P \vdash Q_1\;*\;?_1 \lor Q_2 \;*\; ?_2$, because each of the $P \vdash Q_i$ may not hold.

% This fact 

In most cases, we aim to describe the relevant program state using assertions that are as concise as possible, particularly for loop invariants. However, there are scenarios where more detailed specifications are necessary. For example, in the following case, \lstinline{x} increments to 50, after which both \lstinline{x} and \lstinline{y} increment together to 100.

\begin{lstlisting}
y = 50; x = 0;
while (x < 100) {
    if (x < 50) {
        x++;
    } else {
        x++;
        y++;
    }
}
\end{lstlisting}

A straightforward approach is to define a predicate to describe this process. However, this would generate VCs related to the loop invariant, all of which require manual proofs from the user. From the perspective of user, defining such a predicate and its associated proofs is clearly an unnecessary burden.

% \begin{lstlisting}
%    y == 50 && x == 0 
% |-- 0 <= x <= 100 && 50 <= y <= 100 && incr_50_100(x, y)

%    x < 50 && 0 <= x <= 100 && 50 <= y <= 100 && incr_50_100(x, y)
% |-- 0 <= x + 1 <= 100 && 50 <= y <= 100 && incr_50_100(x + 1, y)

%    x >= 50 && 0 <= x <= 100 && 50 <= y <= 100 && incr_50_100(x, y)
% |-- 0 <= x + 1 <= 100 && 50 <= y + 1 <= 100 && incr_50_100(x + 1, y + 1)
   
% \end{lstlisting}

Another approach is to use a disjunction of assertions to describe the loop invariant. For example, the loop invariant here can be written as \lstinline{0 < x <= 50 && y == 50 || 50 < x <= 100 && x == y}. If a full assertion is provided, everything works smoothly. However, when users attempt to write a disjunction of partial assertions, challenges arise: if the solver cannot automatically determine the frame for certain branches, how should symbolic execution proceed? For this example, the precondition \lstinline{y == 50 && x == 0} clearly does not satisfy the second branch of the loop invariant. As a result, symbolic execution cannot proceed further based on this branch.

To address this, we propose a solution based on multi-branch feature. We require users to assign distinct names to each branch of the loop invariant. Program state transitions are specified using \lstinline{A => B}. For example, in this case, the program state upon entering the loop satisfies only the \lstinline{neq} branch, while the state after the loop satisfies the \lstinline{eq} branch. Initially, we only compute the frame for the \lstinline{neq} branch. Once the transition \lstinline{neq => eq} is detected, we compute the frame for the \lstinline{eq} branch and proceed with symbolic execution for that branch.

\begin{lstlisting}
y = 50; x = 0;
/*@ Inv
        neq: x <= 50 && y == 50;
        eq: 100 >= x > 50 && x == y
        with
        all ==> neq
*/
while (x < 100) {
    if (x < 50) {
        /*@ Branch clear eq */
        x++;
    } else {
        x++;
        y++;
        /*@ neq ==> eq */
    }
}
\end{lstlisting} 

==> Features/Multispec.tex <==
\subsection{Multi-spec derivation}

For a function that requires multiple specifications, our solution is straightforward: we allow each function to have multiple specifications, and users can specify which specification to apply during a function call. Furthermore, we stipulate that only one specification is directly verified from the function body, while the others must be proven derivable from this most rigorous specification. This design also aligns with C syntax, where a function may have multiple declarations but only a single definition—an important property, as our focus is on verifying existing code. We present the concise proof obligation below, intentionally misusing meta-level and logic-level quantifiers and omitting the straightforward proof. \wxw{These generated proof obligations will be exported to Rocq files for subsequent manual verification by users.}


$$
\inferrule
{ \forall \bar{x}'. 
    P'(\bar{x}') \vdash \exists \bar{x}. P(\bar{x}) * ( Q(\bar{x}) {\mathrel{-\mkern-6mu*}} Q'(\bar{x}')) \\
  \forall \bar{x}. \left\{P(\bar{x})\right\}c\left\{Q(\bar{x})\right\} }
{ \forall \bar{x'}. \left\{P'(\bar{x'})\right\}c\left\{Q'(\bar{x'})\right\} }
$$

For example, the \lstinline{high_level_spec} and \lstinline{low_level_spec} shown in Figure~\ref{fig:BSTDelete} can be written in the following form. In this way, during verification of the function \lstinline{tree_delete}, it is only necessary to verify the correctness of \lstinline{low_level_spec} and to prove that \lstinline{high_level_spec} is derivable from it. At the function call site, we provide the annotation \lstinline{/*@ where(spec_name) */} to specify the name of the particular specification.

\vspace{-1.0em}
\begin{minted}[frame=lines]{c}
void delete(struct tree **b, int x)
/*@ high_level_spec <= low_level_spec
  With m
  Require INT_MIN <= x && x <= INT_MAX && store_map( *b, m)
  Ensure store_map( *b, map_delete(x, m)) */;
\end{minted}







==> Features/PartialAssertion.tex <==
\subsection{Partial assertion}\label{fea::pasrt}

Writing out complete assertions is both tedious and error-prone. Instead, we often prefer to specify only the part of the program state that ``changes'', particularly in loop invariants. For example, in the following piece of code, users would prefer not to write out variables that are not modified here. Since the loop only traverses the singly linked list starting from \lstinline{p} using \lstinline{q}, the loop invariant here only needs to concern the shape of the singly linked list involving \lstinline{p} and \lstinline{q}.
\vspace{-1.0em}
\begin{minted}[frame=lines]{c}
...
/*@ listrep(p) */
/*@ Inv lseg(p, q) * listrep(q) */ 
for (struct list *q = p; q != NULL; q = q->next)
    print(q->data);
...
\end{minted}
%The question arises: should the rest of the frame be considered unchanged or "not cared"? We choose the former because it fits realistic situations and admits a clear implementation: each \emph{partial} assertion is complemented using the program state at that point as an elaboration process, rather than being treated as primitive. 
This approach requires the separation-logic solver to be able to infer the frame in an entailment, which our solver supports naturally. For example, assuming the incoming program state \lstinline{n == 0 && p->data == 0 && listrep(p->next) *} \linebreak \lstinline{listrep(r)}, the previous code turns to:


\vspace{-1.0em}
\begin{minted}[frame=lines]{c}
...
/* need-to-solve 
      n == 0 && p->data == 0 && listrep(p->next) * listrep(r)
    |-- ? * listrep(p) */
/*@ Assert exists l, n == 0 && listrep(p) * listrep(r) */
/* need-to-solve 
     q == p && n == 0 && listrep(p) * listrep(r)
   |-- ? * lseg(p, q) * listrep(q) */
/*@ Inv Assert n == 0 && lseg(p, q) * listrep(q) * listrep(r) */ 
for (struct list *q = p; q != NULL; q = q->next)
    print(q->data);
...
\end{minted}



==> Features/UserAssertion.tex <==
\subsection{\wxw{User Assertion Design}}

Our front-end assertion language employs a C-like syntax for enhanced readability, following the design approach of VeriFast. While the translation to separation logic presents non-trivial challenges, the process maintains a rigorous formal definition. To facilitate understanding of subsequent examples, we briefly outline our front-end assertion definition.

%For an automatic verification tool, the most critical step is to successfully perform symbolic execution on annotated C programs and generate VCs. Therefore, the design of the assertion language plays a pivotal role in enabling precise and efficient symbolic execution. Similar to existing verification tools, the assertion language of QCP is based on separation logic. However, it is designed to align more closely with the description habits of the C language. We aim for this design to enable C programmers to become familiar with our tools more quickly and intuitively. 

\begin{figure*}[!ht]
\centering
\vspace{-1.0em}
\begin{tabular}{llcll}
  Expression & $e$ & ::= & $z \in Z$ & integer literal\\
  && \myalt & $v_p$ \myalt $v_l$ & C variable, logic variable\\
  && \myalt & \texttt{\&}$e$ \myalt \texttt{*}$e$ & address, dereference\\
  && \myalt & $\odot e$ \myalt $e_1 \oplus e_2$ & unary and binary operation\\
  && \myalt & $e_1$\texttt{[}$e_2$\texttt{]} & array indexing\\
  && \myalt & $e$\texttt{.}$m$ \myalt $e$\texttt{->}$m$ & member access\\
  && \myalt & \texttt{sizeof}$(t)$\texttt{} & type size\\
  && \myalt & $f(e_1,\ldots,e_n)$ & custom function\\

  Unary operator & $\odot$ & ::= & \texttt{!}\myalt\texttt{\~{}}\myalt\texttt{-}\myalt\texttt{+}\myalt ...\\

  Binary operator & $\oplus$ & ::= & \texttt{+}\myalt\texttt{-}\myalt\texttt{*}\myalt\texttt{/}\myalt ...\\
\end{tabular}
\caption{Syntax of expressions.}
\label{figure:uae}
\vspace{-1.0em}
\end{figure*}

Here, we provide a concise definition of expressions in the form of syntax trees, as illustrated in Figure~\ref{figure:uae}. The design of assertion expressions closely mirrors that of C expressions, ensuring familiarity for developers. The only notable difference is the introduction of custom functions, which operate in the \emph{logic} domain. Users can declare these functions, using the annotation \lstinline{/*@ Extern Coq (f:...)*/}, enabling their use within assertions.


\begin{figure*}
\centering
\begin{tabular}{llcll}
  Pure proposition & $P$ & ::= & $e_1 \oplus e_2$ & comparison\\
  && \myalt & $P_1$\texttt{ \&\& }$P_2$ & conjunction\\
  && \myalt & $P_1$\texttt{ || }$P_2$ & disjunction\\
  && \myalt & $P_1$\texttt{ -> }$P_2$ & implication\\
  && \myalt & \texttt{!}$P$ & negation\\
  && \myalt & \texttt{exists }$x, P$ & existential quantification\\
  && \myalt & \texttt{forall }$x, P$ & universal quantification\\
  && \myalt & $p(e_1,\ldots,e_n)$ & custom predicate\\

  Spatial proposition, assertion & $S$ & ::= & $P$ &\\
  && \myalt & $P$\texttt{ \&\& }$S$ & conjunction\\
  && \myalt & $S_1$\texttt{ * }$S_2$ & separating conjunction\\
  && \myalt & $S_1$\texttt{ || }$S_2$ & disjunction\\
  && \myalt & \texttt{exists }$x, S$ & existential quantification\\
  && \myalt & $p(e_1,\ldots,e_n)$ & custom predicate\\

  Comparison operator & $\oplus$ & ::= & \texttt{>} \myalt \texttt{>=} \myalt \texttt{<} \myalt \texttt{<=} \myalt \texttt{==} \myalt \texttt{!=}
\end{tabular}
\caption{Syntax of user assertions.}
\label{figure:ua}
\end{figure*}

A user assertion can consist of multiple branches, each divided into two sections: one describing pure facts and the other describing memory aspects. The syntax tree for these assertions is defined in Figure~\ref{figure:ua}. The semantics of user assertions differ slightly from textbook separation logic due to their human-computer interaction considerations. For example, QCP allows users to write \lstinline{*y==x->tail}, which is equivalent to:
\begin{small}
\begin{lstlisting}
    exists v yp,
    store((field_addr(x,tail),v) * store(y, yp) * store(yp, v)
\end{lstlisting}
\end{small}

Each proposition—whether pure or spatial—describes such memory locations, along with their spatial components if applicable. When propositions are connected through conjunction (\texttt{\&\&}) or separating conjunction (\texttt{*}), we union these locations; when connected through disjunction (\texttt{||}), we keep them local to each case. Similar to custom functions, users can also define custom predicates. For instance, \lstinline{store_map(p, m)} denotes that a mapping $m$ is stored at the location $p$.

% Based on the definition of user assertions, we can further define the structure of function specifications. The syntax of function specifications is formally defined in Figure~\ref{figure:spec}. A function specification consists of three parts: logical variable list (\textbf{With} clause), precondition (\textbf{Require} clause), and postcondition (\textbf{Ensure} clause).

% \begin{figure*}
% \centering
% \begin{tabular}{llcll}
%   Function specification & $F$ & ::= & $(\forall v_1,\ldots,v_n. S_{pre}, S_{post})$
% \end{tabular}
% \caption{Syntax of function specification.}
% \label{figure:spec}
% \end{figure*}

% \paragraph{\textbf{With clause.}}
% An implicit "$\forall$" around the specification. They are sometimes essential to relate the program state at the function exit point to the one at the function entry. They can even appear in annotations inside the function so that developers have convenient access to the initial state. In general, their values should be "determinable" from the precondition.

% \paragraph{\textbf{Require clause.}}
% The precondition describes properties that the program state at function entry should satisfy.

% \paragraph{\textbf{Ensure clause.}}
% The postcondition describes properties that the program states when the function exits should satisfy. We use the keyword \texttt{\_\_return} to refer to the return value, if any.


==> MotivaExample/Discussion.tex <==
To support C program verification involving memory manipulation, QCP and existing design tools choose to use separation logic as their logic basis, and separation-logic-based symbolic execution enhances automation. However, this symbolic execution process is not guaranteed to succeed unconditionally.

Separation-logic-based symbolic execution identifies and isolates memory regions accessed during load/store operations or function calls. \wxw{For load/store, this requires automatically deriving entailments of the form: \lstinline{P |-- store(x,v) * F}
where \lstinline{store(x,v)} represents the accessed memory cell and \lstinline{F} accounts for the frame assertion.} For function calls, the verifier must similarly find memory regions satisfying the callee's precondition by deriving:
\lstinline{P |--  P_f * F}
where \lstinline{P_f} is the callee's precondition. For this purpose, symbolic heaps (a special form of separation logic assertions, see Fig.~\ref{fig:symbolicheap}) are widely used so that those separating conjuncts \lstinline{store(x,v)} and \lstinline{P_f} mentioned above can hopefully be found atomatically in \lstinline{P} in simple cases and then the frame assertion can be defined by the rest separating conjuncts. For nontrivial cases, effectively solving those entailments above is still challenging in the presence of user-defined predicates, where predicates may require context-aware folding/unfolding.

\begin{figure}
  \centering
  \vspace{-1.0em}
  \begin{minipage}{0.9\linewidth}
    symbolic heap: $(\phi_1 \land \phi_2 \land \cdots \land \phi_n) \land (\psi_1 \ast \psi_2 \ast \cdots \ast \psi_m)$
    
    \vspace{0.5em}
    \begin{tabular}{@{}ll@{}}
      \textbf{where}: & $\phi_i$: non-spatial predicates \\
                      & $\psi_i$: spatial predicates
    \end{tabular}
  \end{minipage}
  \vspace{-1.0em}
  \caption{Single-branch symbolic heap definition following~\cite{10.1007/978-981-96-0602-3_3}.}
  \vspace{-1.0em}
  \label{fig:symbolicheap}
\end{figure}

%In separation-logic-based symbolic execution, assertions are typically represented as \emph{symbolic heaps}—a form that enables efficient spatial reasoning during forward symbolic execution. Following~\cite{10.1007/978-981-96-0602-3_3}, a single-branch symbolic heap can be defined as: $ (\phi_1 \&\& \phi_2 \&\& \cdots \&\& \phi_n) \&\& (\psi_1 * \psi_2 * \cdots * \psi_m) $ where $\phi_i$ denotes non-spatial predicates and $\psi_i$ represents spatial predicates. Unless otherwise specified, all subsequent references to ``single-branch assertions'' in this paper specifically indicate single-branch symbolic heaps.


Existing verification tools achieve high verification efficiency in many examples (many of which are verification-oriented examples) through three carefully designed features:
%Existing verification tools achieve high verification efficiency in many examples through three carefully designed features: 
%Existing verification tools adopt three predominant approaches: fully automated bi-abduction systems (e.g. Infer~\cite{10.5555/1986308.1986345}), annotation-based systems (e.g., VeriFast~\cite{VeriFast}, Viper~\cite{Viper}, and Smallfoot~\cite{10.1007/11804192_6}), and interactive systems (e.g., VST~\cite{VST} using Rocq). These methods achieve high verification efficiency in many examples through three carefully designed features: 
(1) One specification is manually provided for each C function in verification (unless a C function would be inlined in symbolic execution), which enables automatic specification identification and symbolic execution calls. 
(2) Integration of either built-in predicate abduction systems or simple manual control commands to handle separation logic predicate transformations. These assertion transformation systems perform effectively for verification-oriented programs that require only single-branch assertions. Specifically, such manual commands can accurately select the separation conjuncts to be added or deleted, as a separation conjunct will not appear more than once in a single-branch assertion. For instance, \lstinline{store(a,b) * store(a,b)} is always false, and is thus never used in practice. (3) Based on these observations, tools like VST and VeriFast require users to employ only single-branch assertions. This approach offers several advantages: single-branch assertions enable highly efficient symbolic execution, and their transformation requires only simple manual control commands.

When considering real-world C programs, the assumptions underlying these two design considerations do not always hold. We identify two key limitations of the designs above: (1) the single-specification constraint prevents accurate modeling of complex program behaviors, particularly in programs with multiple operational modes or context-dependent invariants; (2) the abstraction of the single-branch symbolic heap, along with existing manual control commands, is insufficient for real-world scenarios that require differentiated operations in distinct branch assertions. Furthermore, we demonstrate that the rule-based operational commands provided by existing tools are insufficient. Several real-world program verification scenarios will be presented to illustrate these limitations.

%These constraints, combined with the requirement to verify unmodified original program code, motivate our core technical contribution: a novel annotation system that is more expressive and capable of supporting such verification styles.

\input{Features/UserAssertion}

==> MotivaExample/MultiBranch.tex <==
\subsection{Single-branch assertion is not enough}\label{motiv::multi}

Existing abduction systems still exhibit significant limitations in reasoning about disjunctions of separation logic assertions. Specifically, they struggle to handle case splitting for single-branch assertions (e.g., \lstinline{A |-- C || D}) and correspondence between multi-branch assertions (e.g., \lstinline{A || B |-- C || D}). However, multi-branch structures are ubiquitous in real-world code, posing major challenges for symbolic execution -- particularly in deriving loop invariants. Below we illustrate these challenges using a representative example from the VST-A~\cite{10.1145/3632911} benchmark.

\begin{figure}[t]
  \centering
  \inputminted[frame=lines,linenos]{c}{Figures/rbt.list}
  \vspace{-1.0em}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{A red-black tree example from VST-A.}
  \vspace{-1.0em}
  \label{fig:rbt}
\end{figure}

Figure~\ref{fig:rbt} illustrates the classic red-black tree insertion balancing algorithm. When the rotation on line 15 executes, the loop terminates immediately because the assignment on line 14 ensures the loop condition will evaluate to false in the next iteration. This behavior creates a verification dilemma - if we specify the loop invariant at line 3 (before condition checking), we must simultaneously capture both the standard bottom-up RBT repair invariant and the special termination case where final rotation completes the repair. A more elegant solution would employ a single invariant at line 5 while separately handling the rotation-triggered exit path. However, mainstream goal-directed verifiers preclude this flexible approach due to their compulsory loop invariant requirements. Although VST-A recognizes this issue, its reliance on manual Coq-based symbolic execution still forces users to provide complete assertions explicitly - an exceptionally onerous requirement for complex algorithms.

If the aforementioned scenario could still be resolved using flexible position loop invariants, the case presented in Figure~\ref{fig:Queue} demonstrates significantly greater complexity. In this example, the memory state represented by parameter \lstinline{bufferAddr} exhibits dependencies on both \lstinline{operateType} and \lstinline{ispointint}. Following the switch statement (line 8), the assertions necessarily develop into intricate multi-branch conditions. When processing subsequent nested statements, each branch's assertion transitions from a single-path condition to a more complex form. Under these conditions, the previously discussed symbolic execution approach for single-path analysis and assertion transformation methods prove inadequate. One might suggest refactoring this function into three separate functions to simplify verification. However, we must verify the current implementation as it exists. The necessity of such modifications to ordinary correct C code remains questionable for enterprise internal development or the open-source community.

\begin{figure}[!htp]
  \centering
  \inputminted[frame=lines,linenos]{c}{Figures/Queue.list}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{OsQueueBufferOperateUpdate from LiteOS.}
  \vspace{-1.0em}
  \label{fig:Queue}
\end{figure}

==> MotivaExample/MultiSpec.tex <==
\subsection{One function specification is not enough}\label{motiv::spec}

In many existing verification tools, one C function is required to have one specification. On the one hand, this specification needs to be verified w.r.t. the C function's implementation. On the other hand, this specification is used in symbolic execution when this C function is triggered. However, in symbolic execution, this approach is sometimes suboptimal or impossible.

This insufficiency becomes particularly evident when comparing high-level predicates with implementation-level predicates. To illustrate this, we consider the deletion operation in a binary search tree used to construct a mapping (See Figure~\ref{fig:BSTDelete}). During the verification of the function \lstinline{delete()}, it is necessary to reason about the specific data structure predicate (e.g., \lstinline{store_tree(x, tr)}, which denotes that pointer x stores a binary search tree tr ). However, when verifying the callers of this function, the primary concern is the existence of the mapping rather than its concrete implementation. Therefore, in this context, we focus exclusively on the higher-level predicate \lstinline{store_map}, abstracting away the implementation details of the mapping. Here \lstinline{store_map(x,m)} indicates that pointer x contains a mapping.

\begin{figure}[t]
  \centering
  \inputminted[frame=lines,linenos]{c}{Figures/tree_delete.list}
  \vspace{-1.0em}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{Binary search tree delete function specifications. Here, \lstinline{store_tree(x, tr)} denotes that pointer x stores a binary search tree tr (defined in Rocq as an inductive type), while \lstinline{store_map(x,m)} indicates that pointer x contains a mapping (defined in Rocq as a total function). The operations \lstinline{tree_delete} and \lstinline{map_delete} remove nodes with specified keys from the tree and mapping respectively.}
  \vspace{-1.0em}
  \label{fig:BSTDelete}
\end{figure}

A proposed methodology advocates for maintaining solely high-level specifications while deferring fold/unfold operations to function verification stages. However, this approach reveals three limitations: (1) Fold operations must propagate through all exit paths. This creates redundancy in functions with multiple return statements. (2) It becomes challenging to establish a unified representation when multiple high-level specifications coexist for the same implementation (e.g., polymorphic lists in OS kernels). (3) Recursive functions demand implementation-level verification prior to high-level specification abstraction.

A more common scenario occurs when a function requires distinct specifications depending on its invocation context. For example, Figure~\ref{fig:LosListDelete} demonstrates a general specification for the \lstinline{LOS_ListDelete} function from LiteOS~\cite{liteos_github}, \wxw{a lightweight operating system based on a real-time kernel}. To simplify the description, we have reduced the original polymorphic doubly-linked list to a circular doubly-linked list where each node stores an integer. The actual verification example still uses the original complex doubly-linked list structure from LiteOS. Unless otherwise specified, all subsequent references to \lstinline{LOS_DL_LIST} pertain to our simplified doubly-linked list structure. Figure~\ref{fig:LOS_DL_LIST} illustrates the simplified definition of \lstinline{LOS_DL_LIST}, which consists of only a previous pointer (\lstinline{pstPrev}), a next pointer (\lstinline{pstNext}), and a data pointer (\lstinline{pstData}).

\begin{figure}[t]
  \centering
  \inputminted[frame=lines,linenos]{c}{Figures/LOS_ListDelete.list}
  \vspace{-1.0em}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{Specification of \lstinline{LOS_ListDelete} from LiteOS. The predicate \lstinline{store_dll(x,l)} represents a circular doubly-linked list storage structure, where \lstinline{x} denotes the sentinel node and \lstinline{l} represents the stored data list.}
  \vspace{-1.0em}
  \label{fig:LosListDelete}
\end{figure}

The predicate \lstinline{store_dll(x,l)} represents a circular doubly-linked list storage structure, where \lstinline{x} denotes the sentinel node and \lstinline{l} represents the stored data list.  To ensure each node in the doubly-linked list remains accessible, the data list stores not only the values of \lstinline{pstData} but also the addresses of corresponding \lstinline{LOS_DL_LIST} nodes. This design guarantees external access to specific nodes and enables sentinel node replacement. 

\begin{figure}[!htp]
  \centering
  \includegraphics[width=1\textwidth]{Figures/DLL.png}
  \vspace{-1.0em}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{The definition of \lstinline{LOS_DL_LIST} in LiteOS. The node \lstinline{x} serves as a sentinel node, and its \lstinline{pstData} field remains unused.}
  \vspace{-1.0em}
  \label{fig:LOS_DL_LIST}
\end{figure}

In the precondition of \lstinline{LOS_ListDelete}, we ensure the membership of the node in the doubly-linked circular list containing \lstinline{x} by partitioning the data list into three segments: \lstinline{l1}, \lstinline{(a,node)}, and \lstinline{l2}. The postcondition guarantees the removal of the specified node by extracting its contents from the modified list structure. This specification accurately describes the function's core functionality - node deletion while maintaining list integrity. However, this specification proves inconvenient for practical invocation scenarios. 

For instance, during operations on the recycle list, every deletion invariably starts from the node immediately following the sentinel node, implying the pre-call program state must always be \lstinline{store_dll(x,cons((a,node),l))}. Conversely, for operations on the pendlist, we only know the target node exists within the list (\lstinline{(a,node)} $\in$ \lstinline{l) && store_dll(x,l)}). Consider the frequency of these invocation patterns, performing assertion transformations before each call becomes prohibitively cumbersome. 

% \paragraph{Multiple specifications}
\wxw{Some verifier developers and maintainers have recognized this fundamental limitation. Frama-C~\cite{Kirchner2015FramaC} allows multiple specifications for functions (referred to as "behaviours"). However, Frama-C is limited to handling cases where each branch is assigned a specific behavior. It cannot address scenarios like \lstinline{delete}, where the derivation between high-level and low-level specifications is required. VSU~\cite{10.1007/978-3-030-72019-3_5} extends VST by constructing comprehensive proofs through modular "verified software units." Between units, exported specifications serve as abstractions of entries via specification subsumption. This mechanism constitutes a form of multiple specification at the modular level. However, VSU's design only supports multiplicity \emph{between} modules, whereas each module internally maintains a single specification. Hip/Sleek~\cite{10.5555/1763048.1763074} advances further by supporting specification derivations. However, their approach mandates automatic solver verification of these derivations - a requirement that becomes untenable for complex functional correctness scenarios. Moreover, during function invocation, these verifiers rely on solvers to automatically select applicable specifications, which may lead to redundant branching and unintended specification selection. Consequently, we propose developing more convenient specifications tailored to these specific cases - a requirement that existing verifiers cannot currently satisfy.}

==> MotivaExample/Operational.tex <==
\subsection{Rule-based operational command is not enough}\label{motiv::operation}

Tools like VeriFast provide mechanisms such as \lstinline{open}/\lstinline{close} commands and lemma functions for manual assertion transformation. However, these approaches present significant usability challenges for typical verification engineers. First, most users lack the expertise to author appropriate lemma functions and construct proofs using C-style syntax. Second, the \lstinline{open}/\lstinline{close} paradigm often proves insufficient for decomposition needs, particularly when predicates admit multiple valid expansion paths. This limitation motivates our proposal for more intuitive annotations to support assertion transformation. To demonstrate this scenario, we also examine functions from LiteOS featuring the \lstinline{LOS_DL_LIST} structure, the system's polymorphic circular doubly-linked list implementation. For clarity in our explanation, we assume the data field contains an integer value.

In our verification of the \lstinline{LOS_ListAdd} operation that inserts a node after a specified position in a doubly linked list, we establish minimal precondition requirements and show in Figure~\ref{fig:LosListAdd}. Specifically, we only require: (1) ownership of the new node's pointer fields (\lstinline{has_permission(&(node->pstPrev))} and \lstinline{has_permission(&(node->pstNext))})\footnote{\wxw{Here, \lstinline{has_permission(x)} indicates that we possess access rights to address \lstinline{x}, regardless of whether its current value is uninitialized or irrelevant to our verification context. This predicate enforces the following memory access discipline: while writing to \lstinline{x} is permitted, reading from \lstinline{x} is only valid after a write operation. From this definition, we directly derive the entailment \lstinline{store(x,v) |-- has_permission(x)}.}}, and (2) permissions for \lstinline{list->pstNext} and the \lstinline{pstPrev} field of the node following the insertion point\footnote{When attempting to acquire full permissions for both x and list, special consideration must be given to the case where \lstinline{x = list}, as this would result in duplicate permission requests and violate separation logic principles.}. This minimal specification is sufficient because we intentionally abstract away the new node's original predecessor/successor relationships and focus solely on the permissions needed for appending after the given \lstinline{list} position.

\begin{figure}[!htp]
  \vspace{-1.0em}
  \centering
  \inputminted[frame=lines,linenos]{c}{Figures/LOS_ListAdd.list}
  \vspace{-1.0em}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{Sepecification of \lstinline{LOS_ListAdd}. The predicate \lstinline{has_permission} describes the ownership of the memory location while treating its contents as an uninitialized value.}
  \label{fig:LosListAdd}
  \vspace{-1.0em}
\end{figure}


Building upon this foundational function, we can formally define two derived operations: \lstinline{LOS_ListHeadInsert} for prepending a node to the head of the list and \lstinline{LOS_ListTailInsert} for appending a node to the tail. Figure~\ref{fig:LosListHeadInsert} and Figure~\ref{fig:LosListTailInsert} shows these functions and relevant specifications.

To enable symbolic execution, we decompose the abstract predicate \lstinline{store_dll(list,l)} into two distinct forms: (1) the form containing \lstinline{list->pstPrev}, \lstinline{list->pstPrev->pstNext}, and the remaining segment (the doubly-linked list from \lstinline{list} to \lstinline{list->pstPrev}); and (2) the form containing \lstinline{list->pstNext}, \lstinline{list->pstNext->pstPrev}, and the remaining segment (the doubly-linked list from \lstinline{list->pstNext} to \lstinline{list}). The conventional open/close operations prove too rigid in this context, as they cannot gracefully handle scenarios requiring dynamic selection of unfolding strategies based on verification contexts. This motivates our design of a more flexible assertion transformation mechanism capable of automatically selecting the most appropriate predicate unfolding form according to the current verification objectives.

\begin{figure}[!htp]
  \vspace{-1.0em}
  \centering
  \inputminted[frame=lines,linenos]{c}{Figures/LOS_ListHeadInsert.list}
  \vspace{-1.0em}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{Sepecifications of \lstinline{LOS_ListHeadInsert}.}
  \vspace{-1.0em}
  \label{fig:LosListHeadInsert}
\end{figure}

\begin{figure}[!htp]
  \vspace{-3.0em}
  \centering
  \inputminted[frame=lines,linenos]{c}{Figures/LOS_ListTailInsert.list}
  \vspace{-1.0em}
  \captionsetup{justification=raggedright, singlelinecheck=false}
  \caption{Sepecifications of \lstinline{LOS_ListTailInsert}.}
  \label{fig:LosListTailInsert}
  \vspace{-3.0em}
\end{figure}

==> Motivation.tex <==
\section{Typical problems in verifying realistic programs}\label{sec::examples}

\input{MotivaExample/Discussion}
\input{MotivaExample/MultiSpec}
\input{MotivaExample/MultiBranch}
\input{MotivaExample/Operational}
